Mal2GCN: A Robust Malware Detection Approach Using Deep Graph Convolutional Networks With Non-Negative Weights

With the growing pace of using Deep Learning (DL) to solve various problems, securing these models against adversaries has become one of the main concerns of researchers. Recent studies have shown that DL-based malware detectors are vulnerable to adversarial examples. An adversary can create carefully crafted adversarial examples to evade DL-based malware detectors. In this paper, we propose Mal2GCN, a robust malware detection model that uses Function Call Graph (FCG) representation of executable files combined with Graph Convolution Network (GCN) to detect Windows malware. Since FCG representation of executable files is more robust than raw byte sequence representation, numerous proposed adversarial example generating methods are ineffective in evading Mal2GCN. Moreover, we use the non-negative training method to transform Mal2GCN to a monotonically non-decreasing function; thereby, it becomes theoretically robust against appending attacks. We then present a black-box source code-based adversarial malware generation approach that can be used to evaluate the robustness of malware detection models against real-world adversaries. The proposed approach injects adversarial codes into the various locations of malware source codes to evade malware detection models. The experiments demonstrate that Mal2GCN with non-negative weights has high accuracy in detecting Windows malware, and it is also robust against adversarial attacks that add benign features to the Malware source code.

==> roc.dat.tex <==
( 0.0 , 0.0 )( 0.004265997490589712 , 0.8731489741302408 )( 0.004265997490589712 , 0.8792149866190901 )( 0.004265997490589712 , 0.8865298840321142 )( 0.004265997490589712 , 0.887778768956289 )( 0.004265997490589712 , 0.8895628902765388 )( 0.004265997490589712 , 0.8900981266726138 )( 0.004265997490589712 , 0.8911685994647636 )( 0.004265997490589712 , 0.8917038358608386 )( 0.004265997490589712 , 0.8929527207850134 )( 0.004265997490589712 , 0.895272078501338 )( 0.004265997490589712 , 0.895985727029438 )( 0.004265997490589712 , 0.8968777876895629 )( 0.004265997490589712 , 0.8972346119536129 )( 0.004265997490589712 , 0.8974130240856378 )( 0.005269761606022585 , 0.8988403211418377 )( 0.005269761606022585 , 0.8993755575379125 )( 0.005269761606022585 , 0.9000892060660125 )( 0.005269761606022585 , 0.9002676181980375 )( 0.005520702634880803 , 0.9004460303300624 )( 0.005771643663739021 , 0.9004460303300624 )( 0.005771643663739021 , 0.9016949152542373 )( 0.005771643663739021 , 0.9022301516503122 )( 0.005771643663739021 , 0.9025869759143622 )( 0.005771643663739021 , 0.9033006244424621 )( 0.005771643663739021 , 0.904371097234612 )( 0.005771643663739021 , 0.9047279214986619 )( 0.005771643663739021 , 0.9052631578947369 )( 0.005771643663739021 , 0.9059768064228367 )( 0.005771643663739021 , 0.9070472792149866 )( 0.005771643663739021 , 0.9079393398751116 )( 0.005771643663739021 , 0.9082961641391615 )( 0.005771643663739021 , 0.9086529884032114 )( 0.005771643663739021 , 0.9088314005352364 )( 0.005771643663739021 , 0.9091882247992864 )( 0.005771643663739021 , 0.9102586975914362 )( 0.005771643663739021 , 0.9106155218554862 )( 0.005771643663739021 , 0.9107939339875112 )( 0.005771643663739021 , 0.9111507582515611 )( 0.005771643663739021 , 0.9113291703835861 )( 0.005771643663739021 , 0.911685994647636 )( 0.005771643663739021 , 0.911864406779661 )( 0.005771643663739021 , 0.9129348795718109 )( 0.005771643663739021 , 0.9131132917038358 )( 0.005771643663739021 , 0.9134701159678859 )( 0.005771643663739021 , 0.9138269402319358 )( 0.00602258469259724 , 0.9138269402319358 )( 0.00602258469259724 , 0.9140053523639607 )( 0.00602258469259724 , 0.9150758251561106 )( 0.00602258469259724 , 0.9157894736842105 )( 0.00602258469259724 , 0.9163247100802855 )( 0.00602258469259724 , 0.9165031222123105 )( 0.00602258469259724 , 0.9168599464763604 )( 0.00602258469259724 , 0.9172167707404103 )( 0.00602258469259724 , 0.9177520071364853 )( 0.00602258469259724 , 0.9184656556645852 )( 0.00602258469259724 , 0.9188224799286352 )( 0.00602258469259724 , 0.9193577163247101 )( 0.006273525721455458 , 0.9193577163247101 )( 0.006273525721455458 , 0.91971454058876 )( 0.006273525721455458 , 0.9200713648528099 )( 0.006273525721455458 , 0.920249776984835 )( 0.006273525721455458 , 0.9207850133809099 )( 0.006273525721455458 , 0.9211418376449598 )( 0.006273525721455458 , 0.9214986619090099 )( 0.006273525721455458 , 0.9222123104371097 )( 0.006273525721455458 , 0.9229259589652097 )( 0.006273525721455458 , 0.9243532560214095 )( 0.006524466750313676 , 0.9243532560214095 )( 0.006524466750313676 , 0.9264942016057092 )( 0.006524466750313676 , 0.9268510258697591 )( 0.006524466750313676 , 0.928099910793934 )( 0.006524466750313676 , 0.928635147190009 )( 0.006524466750313676 , 0.9289919714540589 )( 0.006524466750313676 , 0.9295272078501338 )( 0.006524466750313676 , 0.9323818019625335 )( 0.006775407779171894 , 0.9323818019625335 )( 0.006775407779171894 , 0.9338090990187333 )( 0.006775407779171894 , 0.9345227475468332 )( 0.006775407779171894 , 0.9354148082069581 )( 0.006775407779171894 , 0.9363068688670829 )( 0.006775407779171894 , 0.9368421052631579 )( 0.006775407779171894 , 0.9371989295272078 )( 0.006775407779171894 , 0.9377341659232827 )( 0.007277289836888331 , 0.9377341659232827 )( 0.007277289836888331 , 0.9384478144513827 )( 0.0075282308657465494 , 0.9384478144513827 )( 0.0075282308657465494 , 0.9395182872435326 )( 0.0077791718946047675 , 0.9395182872435326 )( 0.0077791718946047675 , 0.9404103479036574 )( 0.0077791718946047675 , 0.9407671721677074 )( 0.0077791718946047675 , 0.9434433541480821 )( 0.0077791718946047675 , 0.943800178412132 )( 0.0077791718946047675 , 0.943978590544157 )( 0.0077791718946047675 , 0.9443354148082069 )( 0.0077791718946047675 , 0.9450490633363069 )( 0.008030112923462986 , 0.9450490633363069 )( 0.008030112923462986 , 0.9452274754683319 )( 0.008281053952321205 , 0.9452274754683319 )( 0.008281053952321205 , 0.9457627118644067 )( 0.008281053952321205 , 0.9471900089206066 )( 0.008281053952321205 , 0.9479036574487065 )( 0.008531994981179424 , 0.9479036574487065 )( 0.008531994981179424 , 0.9495093666369313 )( 0.008531994981179424 , 0.9498661909009812 )( 0.008531994981179424 , 0.9500446030330062 )( 0.00903387703889586 , 0.9500446030330062 )( 0.00903387703889586 , 0.9509366636931311 )( 0.00903387703889586 , 0.951293487957181 )( 0.00903387703889586 , 0.9527207850133809 )( 0.009284818067754079 , 0.9527207850133809 )( 0.009284818067754079 , 0.9528991971454059 )( 0.009535759096612296 , 0.9528991971454059 )( 0.009535759096612296 , 0.9532560214094559 )( 0.009535759096612296 , 0.9552185548617306 )( 0.009786700125470515 , 0.9552185548617306 )( 0.009786700125470515 , 0.9557537912578056 )( 0.010288582183186951 , 0.9557537912578056 )( 0.01053952321204517 , 0.9557537912578056 )( 0.01053952321204517 , 0.9561106155218555 )( 0.010790464240903387 , 0.9561106155218555 )( 0.010790464240903387 , 0.9564674397859054 )( 0.011292346298619825 , 0.9564674397859054 )( 0.011292346298619825 , 0.9568242640499554 )( 0.011543287327478042 , 0.9568242640499554 )( 0.011543287327478042 , 0.9571810883140054 )( 0.011794228356336261 , 0.9571810883140054 )( 0.011794228356336261 , 0.9586083853702052 )( 0.01204516938519448 , 0.9586083853702052 )( 0.01204516938519448 , 0.9591436217662801 )( 0.012296110414052697 , 0.9591436217662801 )( 0.012296110414052697 , 0.95950044603033 )( 0.012547051442910916 , 0.95950044603033 )( 0.012547051442910916 , 0.959678858162355 )( 0.012797992471769134 , 0.959678858162355 )( 0.012797992471769134 , 0.960035682426405 )( 0.012797992471769134 , 0.960392506690455 )( 0.013048933500627352 , 0.960392506690455 )( 0.013048933500627352 , 0.9607493309545049 )( 0.013048933500627352 , 0.9614629794826048 )( 0.013299874529485571 , 0.9614629794826048 )( 0.013299874529485571 , 0.9636039250669045 )( 0.013801756587202008 , 0.9636039250669045 )( 0.013801756587202008 , 0.9646743978590544 )( 0.014052697616060227 , 0.9646743978590544 )( 0.014052697616060227 , 0.9652096342551294 )( 0.014303638644918444 , 0.9652096342551294 )( 0.014303638644918444 , 0.9653880463871544 )( 0.014554579673776663 , 0.9653880463871544 )( 0.014554579673776663 , 0.9659232827832293 )( 0.015056461731493099 , 0.9659232827832293 )( 0.015056461731493099 , 0.9664585191793041 )( 0.015307402760351318 , 0.9664585191793041 )( 0.015307402760351318 , 0.9671721677074041 )( 0.015558343789209535 , 0.9671721677074041 )( 0.015558343789209535 , 0.967707404103479 )( 0.01606022584692597 , 0.967707404103479 )( 0.01606022584692597 , 0.968242640499554 )( 0.01631116687578419 , 0.968242640499554 )( 0.01631116687578419 , 0.968421052631579 )( 0.01656210790464241 , 0.968421052631579 )( 0.01656210790464241 , 0.9685994647636039 )( 0.017314930991217063 , 0.9685994647636039 )( 0.017314930991217063 , 0.9689562890276538 )( 0.01756587202007528 , 0.9689562890276538 )( 0.01756587202007528 , 0.9694915254237289 )( 0.0178168130489335 , 0.9694915254237289 )( 0.0178168130489335 , 0.9700267618198037 )( 0.018569636135508157 , 0.9700267618198037 )( 0.018569636135508157 , 0.9702051739518287 )( 0.018820577164366373 , 0.9702051739518287 )( 0.018820577164366373 , 0.9703835860838537 )( 0.01907151819322459 , 0.9703835860838537 )( 0.01907151819322459 , 0.9705619982158786 )( 0.020075282308657464 , 0.9705619982158786 )( 0.020577164366373902 , 0.9705619982158786 )( 0.020577164366373902 , 0.9707404103479037 )( 0.02107904642409034 , 0.9707404103479037 )( 0.02107904642409034 , 0.9712756467439786 )( 0.021580928481806774 , 0.9712756467439786 )( 0.021580928481806774 , 0.9718108831400535 )( 0.021831869510664993 , 0.9718108831400535 )( 0.021831869510664993 , 0.9721677074041035 )( 0.02233375156838143 , 0.9721677074041035 )( 0.02233375156838143 , 0.9727029438001784 )( 0.02258469259723965 , 0.9727029438001784 )( 0.02258469259723965 , 0.9728813559322034 )( 0.023086574654956084 , 0.9728813559322034 )( 0.023086574654956084 , 0.9730597680642283 )( 0.023588456712672522 , 0.9730597680642283 )( 0.023588456712672522 , 0.9734165923282784 )( 0.02383939774153074 , 0.9734165923282784 )( 0.02383939774153074 , 0.9735950044603033 )( 0.024843161856963614 , 0.9735950044603033 )( 0.024843161856963614 , 0.9737734165923283 )( 0.025094102885821833 , 0.9737734165923283 )( 0.025094102885821833 , 0.9743086529884032 )( 0.025595984943538267 , 0.9743086529884032 )( 0.025595984943538267 , 0.9750223015165032 )( 0.026097867001254705 , 0.9750223015165032 )( 0.026097867001254705 , 0.9752007136485281 )( 0.026599749058971143 , 0.9752007136485281 )( 0.027101631116687577 , 0.9752007136485281 )( 0.027101631116687577 , 0.9753791257805531 )( 0.027101631116687577 , 0.975735950044603 )( 0.027101631116687577 , 0.975914362176628 )( 0.027352572145545796 , 0.975914362176628 )( 0.027854454203262234 , 0.975914362176628 )( 0.027854454203262234 , 0.976271186440678 )( 0.028105395232120453 , 0.976271186440678 )( 0.028105395232120453 , 0.976449598572703 )( 0.028607277289836888 , 0.976449598572703 )( 0.028607277289836888 , 0.9768064228367529 )( 0.028858218318695106 , 0.9768064228367529 )( 0.028858218318695106 , 0.9769848349687779 )( 0.029360100376411544 , 0.9769848349687779 )( 0.029360100376411544 , 0.9775200713648529 )( 0.02986198243412798 , 0.9775200713648529 )( 0.02986198243412798 , 0.9778768956289028 )( 0.030614805520702636 , 0.9778768956289028 )( 0.030614805520702636 , 0.9780553077609278 )( 0.030865746549560855 , 0.9780553077609278 )( 0.030865746549560855 , 0.9782337198929527 )( 0.030865746549560855 , 0.9785905441570026 )( 0.03136762860727729 , 0.9785905441570026 )( 0.03136762860727729 , 0.9787689562890276 )( 0.03237139272271016 , 0.9787689562890276 )( 0.03237139272271016 , 0.9789473684210527 )( 0.03262233375156838 , 0.9789473684210527 )( 0.03262233375156838 , 0.9791257805530776 )( 0.03312421580928482 , 0.9791257805530776 )( 0.03312421580928482 , 0.9794826048171276 )( 0.033626097867001256 , 0.9794826048171276 )( 0.033626097867001256 , 0.9796610169491525 )( 0.034127979924717694 , 0.9796610169491525 )( 0.034629861982434125 , 0.9796610169491525 )( 0.03513174404015056 , 0.9796610169491525 )( 0.035633626097867 , 0.9796610169491525 )( 0.035633626097867 , 0.9800178412132025 )( 0.03588456712672522 , 0.9800178412132025 )( 0.03588456712672522 , 0.9807314897413024 )( 0.03613550815558344 , 0.9807314897413024 )( 0.03613550815558344 , 0.9812667261373773 )( 0.036888331242158096 , 0.9812667261373773 )( 0.03814303638644918 , 0.9812667261373773 )( 0.03864491844416562 , 0.9812667261373773 )( 0.03864491844416562 , 0.9814451382694023 )( 0.03889585947302384 , 0.9814451382694023 )( 0.03889585947302384 , 0.9816235504014273 )( 0.03889585947302384 , 0.9819803746654773 )( 0.0396486825595985 , 0.9819803746654773 )( 0.0396486825595985 , 0.9823371989295272 )( 0.04040150564617315 , 0.9823371989295272 )( 0.04040150564617315 , 0.9825156110615522 )( 0.04215809284818068 , 0.9825156110615522 )( 0.04215809284818068 , 0.9828724353256021 )( 0.04341279799247177 , 0.9828724353256021 )( 0.04341279799247177 , 0.9830508474576272 )( 0.0451693851944793 , 0.9830508474576272 )( 0.0451693851944793 , 0.9832292595896521 )( 0.04918444165621079 , 0.9832292595896521 )( 0.04918444165621079 , 0.983586083853702 )( 0.049937264742785446 , 0.983586083853702 )( 0.050439146800501884 , 0.983586083853702 )( 0.05094102885821832 , 0.983586083853702 )( 0.05244667503136763 , 0.983586083853702 )( 0.05244667503136763 , 0.983764495985727 )( 0.053701380175658724 , 0.983764495985727 )( 0.053701380175658724 , 0.983942908117752 )( 0.05846925972396487 , 0.983942908117752 )( 0.05846925972396487 , 0.9841213202497769 )( 0.060225846925972396 , 0.9841213202497769 )( 0.060225846925972396 , 0.984299732381802 )( 0.06097867001254705 , 0.984299732381802 )( 0.06148055207026349 , 0.984299732381802 )( 0.06424090338770388 , 0.984299732381802 )( 0.06424090338770388 , 0.9846565566458519 )( 0.0657465495608532 , 0.9846565566458519 )( 0.0657465495608532 , 0.9848349687778769 )( 0.06624843161856964 , 0.9848349687778769 )( 0.06624843161856964 , 0.9850133809099019 )( 0.06675031367628607 , 0.9850133809099019 )( 0.06725219573400251 , 0.9850133809099019 )( 0.07076537013801756 , 0.9850133809099019 )( 0.07076537013801756 , 0.9853702051739518 )( 0.07151819322459223 , 0.9853702051739518 )( 0.07151819322459223 , 0.9855486173059768 )( 0.07176913425345044 , 0.9855486173059768 )( 0.07227101631116688 , 0.9855486173059768 )( 0.07277289836888332 , 0.9855486173059768 )( 0.07277289836888332 , 0.9857270294380018 )( 0.07728983688833124 , 0.9857270294380018 )( 0.07728983688833124 , 0.9859054415700268 )( 0.07854454203262233 , 0.9859054415700268 )( 0.07854454203262233 , 0.9860838537020518 )( 0.07879548306148056 , 0.9860838537020518 )( 0.0795483061480552 , 0.9860838537020518 )( 0.08030112923462986 , 0.9860838537020518 )( 0.08030112923462986 , 0.9862622658340767 )( 0.08180677540777917 , 0.9862622658340767 )( 0.08180677540777917 , 0.9864406779661017 )( 0.08456712672521957 , 0.9864406779661017 )( 0.08582183186951066 , 0.9869759143621766 )( 0.09360100376411544 , 0.9869759143621766 )( 0.09360100376411544 , 0.9871543264942017 )( 0.09485570890840653 , 0.9871543264942017 )( 0.09485570890840653 , 0.9873327386262266 )( 0.09661229611041405 , 0.9873327386262266 )( 0.09661229611041405 , 0.9875111507582516 )( 0.09786700125470514 , 0.9875111507582516 )( 0.09786700125470514 , 0.9876895628902765 )( 0.0986198243412798 , 0.9876895628902765 )( 0.0986198243412798 , 0.9878679750223015 )( 0.1001254705144291 , 0.9878679750223015 )( 0.1001254705144291 , 0.9880463871543265 )( 0.10062735257214554 , 0.9880463871543265 )( 0.10112923462986198 , 0.9880463871543265 )( 0.1013801756587202 , 0.9880463871543265 )( 0.1013801756587202 , 0.9882247992863514 )( 0.10213299874529486 , 0.9882247992863514 )( 0.10213299874529486 , 0.9884032114183765 )( 0.1028858218318695 , 0.9884032114183765 )( 0.10338770388958594 , 0.9884032114183765 )( 0.10639899623588457 , 0.9884032114183765 )( 0.10639899623588457 , 0.9885816235504015 )( 0.10941028858218318 , 0.9885816235504015 )( 0.10991217063989962 , 0.9885816235504015 )( 0.11267252195734002 , 0.9885816235504015 )( 0.11317440401505646 , 0.9885816235504015 )( 0.11417816813048934 , 0.9885816235504015 )( 0.11417816813048934 , 0.9887600356824264 )( 0.11468005018820578 , 0.9887600356824264 )( 0.11468005018820578 , 0.9889384478144514 )( 0.11744040150564618 , 0.9889384478144514 )( 0.11819322459222083 , 0.9889384478144514 )( 0.11969887076537014 , 0.9889384478144514 )( 0.12020075282308658 , 0.9889384478144514 )( 0.12446675031367628 , 0.9889384478144514 )( 0.12446675031367628 , 0.9892952720785013 )( 0.12823086574654957 , 0.9892952720785013 )( 0.12823086574654957 , 0.9894736842105263 )( 0.12973651191969887 , 0.9894736842105263 )( 0.1302383939774153 , 0.9894736842105263 )( 0.13124215809284817 , 0.9894736842105263 )( 0.13174404015056462 , 0.9894736842105263 )( 0.13324968632371392 , 0.9894736842105263 )( 0.13400250941028857 , 0.9894736842105263 )( 0.13776662484316185 , 0.9894736842105263 )( 0.13776662484316185 , 0.9896520963425512 )( 0.13902132998745295 , 0.9896520963425512 )( 0.13902132998745295 , 0.9898305084745763 )( 0.14153074027603513 , 0.9898305084745763 )( 0.14153074027603513 , 0.9900089206066013 )( 0.14755332496863238 , 0.9900089206066013 )( 0.14855708908406526 , 0.9903657448706512 )( 0.15307402760351319 , 0.9903657448706512 )( 0.15307402760351319 , 0.9905441570026762 )( 0.15633626097867 , 0.9905441570026762 )( 0.15633626097867 , 0.9907225691347011 )( 0.15708908406524466 , 0.9907225691347011 )( 0.1575909661229611 , 0.9907225691347011 )( 0.16110414052697616 , 0.9907225691347011 )( 0.16260978670012546 , 0.9907225691347011 )( 0.16537013801756587 , 0.9907225691347011 )( 0.16612296110414052 , 0.9907225691347011 )( 0.16662484316185697 , 0.9907225691347011 )( 0.16662484316185697 , 0.9909009812667261 )( 0.17038895859473024 , 0.9909009812667261 )( 0.17038895859473024 , 0.9910793933987511 )( 0.17089084065244667 , 0.9910793933987511 )( 0.17089084065244667 , 0.9912578055307761 )( 0.17340025094102887 , 0.9912578055307761 )( 0.17340025094102887 , 0.9914362176628011 )( 0.17691342534504392 , 0.9914362176628011 )( 0.17691342534504392 , 0.991793041926851 )( 0.1779171894604768 , 0.991793041926851 )( 0.1779171894604768 , 0.991971454058876 )( 0.17992471769134252 , 0.991971454058876 )( 0.17992471769134252 , 0.992149866190901 )( 0.1821831869510665 , 0.992149866190901 )( 0.18293601003764115 , 0.992149866190901 )( 0.19096612296110413 , 0.992149866190901 )( 0.1917189460476788 , 0.9923282783229259 )( 0.19498117942283563 , 0.9923282783229259 )( 0.19498117942283563 , 0.992506690454951 )( 0.19799247176913426 , 0.992506690454951 )( 0.19799247176913426 , 0.992685102586976 )( 0.19974905897114179 , 0.992685102586976 )( 0.2002509410288582 , 0.992685102586976 )( 0.2040150564617315 , 0.992685102586976 )( 0.2040150564617315 , 0.9928635147190009 )( 0.20501882057716436 , 0.9928635147190009 )( 0.20501882057716436 , 0.9930419268510259 )( 0.20627352572145546 , 0.9930419268510259 )( 0.2067754077791719 , 0.9930419268510259 )( 0.20903387703889587 , 0.9930419268510259 )( 0.2095357590966123 , 0.9930419268510259 )( 0.21028858218318694 , 0.9930419268510259 )( 0.21028858218318694 , 0.9932203389830508 )( 0.2120451693851945 , 0.9932203389830508 )( 0.2120451693851945 , 0.9933987511150758 )( 0.21279799247176914 , 0.9933987511150758 )( 0.2135508155583438 , 0.9933987511150758 )( 0.2135508155583438 , 0.9935771632471008 )( 0.21656210790464242 , 0.9935771632471008 )( 0.22107904642409035 , 0.9935771632471008 )( 0.22434127979924717 , 0.9935771632471008 )( 0.22434127979924717 , 0.9937555753791257 )( 0.22509410288582182 , 0.9937555753791257 )( 0.22534504391468005 , 0.9939339875111508 )( 0.22936010037641155 , 0.9939339875111508 )( 0.22986198243412798 , 0.9939339875111508 )( 0.23111668757841908 , 0.9939339875111508 )( 0.2316185696361355 , 0.9939339875111508 )( 0.23462986198243413 , 0.9939339875111508 )( 0.23462986198243413 , 0.9941123996431758 )( 0.23889585947302383 , 0.9941123996431758 )( 0.23889585947302383 , 0.9942908117752007 )( 0.23939774153074028 , 0.9942908117752007 )( 0.2529485570890841 , 0.9942908117752007 )( 0.2529485570890841 , 0.9948260481712756 )( 0.25395232120451694 , 0.9948260481712756 )( 0.2544542032622334 , 0.9948260481712756 )( 0.2584692597239649 , 0.9950044603033006 )( 0.25972396486825594 , 0.9950044603033006 )( 0.25972396486825594 , 0.9953612845673506 )( 0.26750313676286075 , 0.9953612845673506 )( 0.26750313676286075 , 0.9955396966993756 )( 0.271267252195734 , 0.9955396966993756 )( 0.271267252195734 , 0.9957181088314006 )( 0.27176913425345045 , 0.9957181088314006 )( 0.2740276035131744 , 0.9957181088314006 )( 0.27452948557089085 , 0.9957181088314006 )( 0.27628607277289835 , 0.9957181088314006 )( 0.27628607277289835 , 0.9958965209634255 )( 0.28431618569636136 , 0.9958965209634255 )( 0.28557089084065246 , 0.9958965209634255 )( 0.2946047678795483 , 0.9958965209634255 )( 0.2946047678795483 , 0.9960749330954505 )( 0.3081555834378921 , 0.9960749330954505 )( 0.3081555834378921 , 0.9962533452274754 )( 0.3111668757841907 , 0.9962533452274754 )( 0.31217063989962357 , 0.9962533452274754 )( 0.3252195734002509 , 0.9962533452274754 )( 0.3252195734002509 , 0.9964317573595004 )( 0.3254705144291092 , 0.9964317573595004 )( 0.3254705144291092 , 0.9966101694915255 )( 0.32772898368883313 , 0.9966101694915255 )( 0.32772898368883313 , 0.9967885816235504 )( 0.3337515683814304 , 0.9967885816235504 )( 0.3342534504391468 , 0.9967885816235504 )( 0.3397741530740276 , 0.9967885816235504 )( 0.3397741530740276 , 0.9969669937555754 )( 0.3462986198243413 , 0.9969669937555754 )( 0.3475533249686324 , 0.9969669937555754 )( 0.3508155583437892 , 0.9969669937555754 )( 0.35131744040150564 , 0.9969669937555754 )( 0.3518193224592221 , 0.9969669937555754 )( 0.35232120451693855 , 0.9969669937555754 )( 0.35834378920953575 , 0.9969669937555754 )( 0.358594730238394 , 0.9971454058876004 )( 0.35984943538268505 , 0.9971454058876004 )( 0.3603513174404015 , 0.9971454058876004 )( 0.36336260978670015 , 0.9971454058876004 )( 0.36336260978670015 , 0.9973238180196253 )( 0.36511919698870765 , 0.9973238180196253 )( 0.36637390213299875 , 0.9973238180196253 )( 0.36637390213299875 , 0.9975022301516503 )( 0.36762860727728985 , 0.9975022301516503 )( 0.3686323713927227 , 0.9975022301516503 )( 0.37641154328732745 , 0.9975022301516503 )( 0.3769134253450439 , 0.9975022301516503 )( 0.37992471769134256 , 0.9975022301516503 )( 0.3806775407779172 , 0.9975022301516503 )( 0.38444165621079046 , 0.9975022301516503 )( 0.3849435382685069 , 0.9975022301516503 )( 0.39974905897114177 , 0.9975022301516503 )( 0.40100376411543287 , 0.9975022301516503 )( 0.4027603513174404 , 0.9975022301516503 )( 0.4032622333751568 , 0.9975022301516503 )( 0.40401505646173147 , 0.9975022301516503 )( 0.40526976160602257 , 0.9975022301516503 )( 0.4117942283563363 , 0.9975022301516503 )( 0.4117942283563363 , 0.9976806422836753 )( 0.41530740276035133 , 0.9976806422836753 )( 0.416060225846926 , 0.9976806422836753 )( 0.41982434127979923 , 0.9976806422836753 )( 0.4203262233375157 , 0.9976806422836753 )( 0.4228356336260979 , 0.9976806422836753 )( 0.42358845671267253 , 0.9976806422836753 )( 0.4406524466750314 , 0.9976806422836753 )( 0.4406524466750314 , 0.9978590544157002 )( 0.4411543287327478 , 0.9978590544157002 )( 0.4411543287327478 , 0.9980374665477253 )( 0.44366373902133 , 0.9980374665477253 )( 0.44366373902133 , 0.9982158786797503 )( 0.44742785445420324 , 0.9982158786797503 )( 0.4481806775407779 , 0.9982158786797503 )( 0.45972396486825595 , 0.9982158786797503 )( 0.4604767879548306 , 0.9982158786797503 )( 0.46800501882057716 , 0.9982158786797503 )( 0.4687578419071518 , 0.9982158786797503 )( 0.46925972396486826 , 0.9982158786797503 )( 0.4697616060225847 , 0.9982158786797503 )( 0.4700125470514429 , 0.9982158786797503 )( 0.47051442910915936 , 0.9982158786797503 )( 0.5036386449184441 , 0.9982158786797503 )( 0.5041405269761606 , 0.9982158786797503 )( 0.5063989962358846 , 0.9982158786797503 )( 0.506900878293601 , 0.9982158786797503 )( 0.5076537013801756 , 0.9982158786797503 )( 0.5081555834378921 , 0.9982158786797503 )( 0.5096612296110414 , 0.9982158786797503 )( 0.5101631116687578 , 0.9982158786797503 )( 0.5146800501882057 , 0.9982158786797503 )( 0.5176913425345044 , 0.9982158786797503 )( 0.5181932245922208 , 0.9982158786797503 )( 0.5214554579673777 , 0.9982158786797503 )( 0.5224592220828106 , 0.9982158786797503 )( 0.526474278544542 , 0.9982158786797503 )( 0.5274780426599749 , 0.9989295272078501 )( 0.5365119196988708 , 0.9989295272078501 )( 0.5370138017565872 , 0.9989295272078501 )( 0.5380175658720201 , 0.9989295272078501 )( 0.5380175658720201 , 0.9991079393398751 )( 0.5417816813048933 , 0.9991079393398751 )( 0.5422835633626097 , 0.9991079393398751 )( 0.5485570890840652 , 0.9991079393398751 )( 0.5500627352572146 , 0.9991079393398751 )( 0.5573400250941029 , 0.9991079393398751 )( 0.5578419071518194 , 0.9991079393398751 )( 0.5606022584692597 , 0.9991079393398751 )( 0.5613550815558344 , 0.9991079393398751 )( 0.5618569636135509 , 0.9991079393398751 )( 0.5636135508155583 , 0.9991079393398751 )( 0.5641154328732748 , 0.9991079393398751 )( 0.5651191969887076 , 0.9991079393398751 )( 0.566624843161857 , 0.9991079393398751 )( 0.570138017565872 , 0.9991079393398751 )( 0.5706398996235884 , 0.9991079393398751 )( 0.5877038895859473 , 0.9991079393398751 )( 0.5882057716436637 , 0.9991079393398751 )( 0.5937264742785445 , 0.9991079393398751 )( 0.594228356336261 , 0.9991079393398751 )( 0.5949811794228357 , 0.9991079393398751 )( 0.5954830614805521 , 0.9991079393398751 )( 0.6070263488080301 , 0.9991079393398751 )( 0.6075282308657466 , 0.9991079393398751 )( 0.609284818067754 , 0.9991079393398751 )( 0.6097867001254705 , 0.9991079393398751 )( 0.613801756587202 , 0.9991079393398751 )( 0.6143036386449184 , 0.9991079393398751 )( 0.6158092848180677 , 0.9991079393398751 )( 0.6163111668757842 , 0.9991079393398751 )( 0.6183186951066499 , 0.9991079393398751 )( 0.6183186951066499 , 0.9992863514719 )( 0.6268506900878293 , 0.9992863514719 )( 0.6283563362609786 , 0.9992863514719 )( 0.6288582183186952 , 0.9992863514719 )( 0.6358845671267253 , 0.9992863514719 )( 0.6393977415307402 , 0.9992863514719 )( 0.6466750313676286 , 0.9992863514719 )( 0.6466750313676286 , 0.9994647636039251 )( 0.6474278544542033 , 0.9994647636039251 )( 0.6479297365119197 , 0.9994647636039251 )( 0.6690087829360101 , 0.9994647636039251 )( 0.6695106649937265 , 0.9994647636039251 )( 0.6777917189460477 , 0.9994647636039251 )( 0.6782936010037641 , 0.9994647636039251 )( 0.6858218318695106 , 0.9994647636039251 )( 0.6863237139272271 , 0.9994647636039251 )( 0.6928481806775407 , 0.9994647636039251 )( 0.6936010037641155 , 0.9994647636039251 )( 0.6963613550815558 , 0.9994647636039251 )( 0.6968632371392722 , 0.9994647636039251 )( 0.6978670012547051 , 0.9994647636039251 )( 0.7189460476787954 , 0.9994647636039251 )( 0.719447929736512 , 0.9994647636039251 )( 0.7239648682559598 , 0.9994647636039251 )( 0.7247176913425345 , 0.9994647636039251 )( 0.736762860727729 , 0.9994647636039251 )( 0.7375156838143037 , 0.9994647636039251 )( 0.7412797992471769 , 0.9994647636039251 )( 0.7417816813048933 , 0.9994647636039251 )( 0.7445420326223338 , 0.9994647636039251 )( 0.7455457967377667 , 0.9994647636039251 )( 0.7535759096612296 , 0.9994647636039251 )( 0.7540777917189461 , 0.9994647636039251 )( 0.7590966122961104 , 0.9994647636039251 )( 0.7595984943538269 , 0.9994647636039251 )( 0.7658720200752823 , 0.9994647636039251 )( 0.7663739021329987 , 0.9994647636039251 )( 0.7691342534504392 , 0.9994647636039251 )( 0.7696361355081556 , 0.9994647636039251 )( 0.7708908406524467 , 0.9994647636039251 )( 0.7708908406524467 , 0.9996431757359501 )( 0.7756587202007528 , 0.9996431757359501 )( 0.7761606022584693 , 0.9996431757359501 )( 0.7831869510664994 , 0.9996431757359501 )( 0.7836888331242158 , 0.9996431757359501 )( 0.8145545796737766 , 0.9996431757359501 )( 0.8150564617314932 , 0.9996431757359501 )( 0.8336260978670013 , 0.9996431757359501 )( 0.8343789209535759 , 0.9996431757359501 )( 0.8361355081555835 , 0.9996431757359501 )( 0.8366373902132999 , 0.9996431757359501 )( 0.8466750313676286 , 0.9996431757359501 )( 0.8471769134253451 , 0.9996431757359501 )( 0.8486825595984944 , 0.9996431757359501 )( 0.8491844416562108 , 0.9996431757359501 )( 0.849435382685069 , 0.9996431757359501 )( 0.849435382685069 , 0.999821587867975 )( 0.852948557089084 , 0.999821587867975 )( 0.8537013801756588 , 0.999821587867975 )( 0.8617314930991217 , 0.999821587867975 )( 0.8617314930991217 , 1.0 )( 0.8737766624843162 , 1.0 )( 0.8742785445420326 , 1.0 )( 0.8755332496863237 , 1.0 )( 0.8765370138017566 , 1.0 )( 0.880552070263488 , 1.0 )( 0.8813048933500628 , 1.0 )( 0.8860727728983688 , 1.0 )( 0.8865746549560853 , 1.0 )( 0.88732747804266 , 1.0 )( 0.8878293601003764 , 1.0 )( 0.888582183186951 , 1.0 )( 0.8900878293601003 , 1.0 )( 0.895357590966123 , 1.0 )( 0.8963613550815558 , 1.0 )( 0.896612296110414 , 1.0 )( 0.8971141781681304 , 1.0 )( 0.9041405269761607 , 1.0 )( 0.904642409033877 , 1.0 )( 0.9111668757841908 , 1.0 )( 0.9116687578419072 , 1.0 )( 0.9227101631116688 , 1.0 )( 0.9232120451693852 , 1.0 )( 0.9249686323713927 , 1.0 )( 0.9254705144291092 , 1.0 )( 0.9304893350062735 , 1.0 )( 0.9312421580928482 , 1.0 )( 0.9322459222082811 , 1.0 )( 0.9327478042659975 , 1.0 )( 0.933249686323714 , 1.0 )( 0.9337515683814304 , 1.0 )( 0.9375156838143036 , 1.0 )( 0.9380175658720201 , 1.0 )( 0.9407779171894605 , 1.0 )( 0.9412797992471769 , 1.0 )( 0.9415307402760351 , 1.0 )( 0.942534504391468 , 1.0 )( 0.9432873274780427 , 1.0 )( 0.9440401505646173 , 1.0 )( 0.9450439146800502 , 1.0 )( 0.9490589711417817 , 1.0 )( 0.9495608531994981 , 1.0 )( 0.954077791718946 , 1.0 )( 0.9545796737766625 , 1.0 )( 0.9683814303638645 , 1.0 )( 0.9693851944792974 , 1.0 )( 0.970138017565872 , 1.0 )( 0.9708908406524467 , 1.0 )( 0.9726474278544542 , 1.0 )( 0.9734002509410289 , 1.0 )( 0.9774153074027604 , 1.0 )( 0.978168130489335 , 1.0 )( 0.9794228356336261 , 1.0 )( 0.9799247176913425 , 1.0 )( 0.9856963613550815 , 1.0 )( 0.986198243412798 , 1.0 )( 0.9914680050188206 , 1.0 )( 0.991969887076537 , 1.0 )( 0.9974905897114178 , 1.0 )( 1.0 , 1.0 ) 

==> roc.tex <==
( 0.0 , 0.0 )( 0.004265997490589712 , 0.8731489741302408 )( 0.004265997490589712 , 0.8792149866190901 )( 0.004265997490589712 , 0.8865298840321142 )( 0.004265997490589712 , 0.887778768956289 )( 0.004265997490589712 , 0.8895628902765388 )( 0.004265997490589712 , 0.8900981266726138 )( 0.004265997490589712 , 0.8911685994647636 )( 0.004265997490589712 , 0.8917038358608386 )( 0.004265997490589712 , 0.8929527207850134 )( 0.004265997490589712 , 0.895272078501338 )( 0.004265997490589712 , 0.895985727029438 )( 0.004265997490589712 , 0.8968777876895629 )( 0.004265997490589712 , 0.8972346119536129 )( 0.004265997490589712 , 0.8974130240856378 )( 0.005269761606022585 , 0.8988403211418377 )( 0.005269761606022585 , 0.8993755575379125 )( 0.005269761606022585 , 0.9000892060660125 )( 0.005269761606022585 , 0.9002676181980375 )( 0.005520702634880803 , 0.9004460303300624 )( 0.005771643663739021 , 0.9004460303300624 )( 0.005771643663739021 , 0.9016949152542373 )( 0.005771643663739021 , 0.9022301516503122 )( 0.005771643663739021 , 0.9025869759143622 )( 0.005771643663739021 , 0.9033006244424621 )( 0.005771643663739021 , 0.904371097234612 )( 0.005771643663739021 , 0.9047279214986619 )( 0.005771643663739021 , 0.9052631578947369 )( 0.005771643663739021 , 0.9059768064228367 )( 0.005771643663739021 , 0.9070472792149866 )( 0.005771643663739021 , 0.9079393398751116 )( 0.005771643663739021 , 0.9082961641391615 )( 0.005771643663739021 , 0.9086529884032114 )( 0.005771643663739021 , 0.9088314005352364 )( 0.005771643663739021 , 0.9091882247992864 )( 0.005771643663739021 , 0.9102586975914362 )( 0.005771643663739021 , 0.9106155218554862 )( 0.005771643663739021 , 0.9107939339875112 )( 0.005771643663739021 , 0.9111507582515611 )( 0.005771643663739021 , 0.9113291703835861 )( 0.005771643663739021 , 0.911685994647636 )( 0.005771643663739021 , 0.911864406779661 )( 0.005771643663739021 , 0.9129348795718109 )( 0.005771643663739021 , 0.9131132917038358 )( 0.005771643663739021 , 0.9134701159678859 )( 0.005771643663739021 , 0.9138269402319358 )( 0.00602258469259724 , 0.9138269402319358 )( 0.00602258469259724 , 0.9140053523639607 )( 0.00602258469259724 , 0.9150758251561106 )( 0.00602258469259724 , 0.9157894736842105 )( 0.00602258469259724 , 0.9163247100802855 )( 0.00602258469259724 , 0.9165031222123105 )( 0.00602258469259724 , 0.9168599464763604 )( 0.00602258469259724 , 0.9172167707404103 )( 0.00602258469259724 , 0.9177520071364853 )( 0.00602258469259724 , 0.9184656556645852 )( 0.00602258469259724 , 0.9188224799286352 )( 0.00602258469259724 , 0.9193577163247101 )( 0.006273525721455458 , 0.9193577163247101 )( 0.006273525721455458 , 0.91971454058876 )( 0.006273525721455458 , 0.9200713648528099 )( 0.006273525721455458 , 0.920249776984835 )( 0.006273525721455458 , 0.9207850133809099 )( 0.006273525721455458 , 0.9211418376449598 )( 0.006273525721455458 , 0.9214986619090099 )( 0.006273525721455458 , 0.9222123104371097 )( 0.006273525721455458 , 0.9229259589652097 )( 0.006273525721455458 , 0.9243532560214095 )( 0.006524466750313676 , 0.9243532560214095 )( 0.006524466750313676 , 0.9264942016057092 )( 0.006524466750313676 , 0.9268510258697591 )( 0.006524466750313676 , 0.928099910793934 )( 0.006524466750313676 , 0.928635147190009 )( 0.006524466750313676 , 0.9289919714540589 )( 0.006524466750313676 , 0.9295272078501338 )( 0.006524466750313676 , 0.9323818019625335 )( 0.006775407779171894 , 0.9323818019625335 )( 0.006775407779171894 , 0.9338090990187333 )( 0.006775407779171894 , 0.9345227475468332 )( 0.006775407779171894 , 0.9354148082069581 )( 0.006775407779171894 , 0.9363068688670829 )( 0.006775407779171894 , 0.9368421052631579 )( 0.006775407779171894 , 0.9371989295272078 )( 0.006775407779171894 , 0.9377341659232827 )( 0.007277289836888331 , 0.9377341659232827 )( 0.007277289836888331 , 0.9384478144513827 )( 0.0075282308657465494 , 0.9384478144513827 )( 0.0075282308657465494 , 0.9395182872435326 )( 0.0077791718946047675 , 0.9395182872435326 )( 0.0077791718946047675 , 0.9404103479036574 )( 0.0077791718946047675 , 0.9407671721677074 )( 0.0077791718946047675 , 0.9434433541480821 )( 0.0077791718946047675 , 0.943800178412132 )( 0.0077791718946047675 , 0.943978590544157 )( 0.0077791718946047675 , 0.9443354148082069 )( 0.0077791718946047675 , 0.9450490633363069 )( 0.008030112923462986 , 0.9450490633363069 )( 0.008030112923462986 , 0.9452274754683319 )( 0.008281053952321205 , 0.9452274754683319 )( 0.008281053952321205 , 0.9457627118644067 )( 0.008281053952321205 , 0.9471900089206066 )( 0.008281053952321205 , 0.9479036574487065 )( 0.008531994981179424 , 0.9479036574487065 )( 0.008531994981179424 , 0.9495093666369313 )( 0.008531994981179424 , 0.9498661909009812 )( 0.008531994981179424 , 0.9500446030330062 )( 0.00903387703889586 , 0.9500446030330062 )( 0.00903387703889586 , 0.9509366636931311 )( 0.00903387703889586 , 0.951293487957181 )( 0.00903387703889586 , 0.9527207850133809 )( 0.009284818067754079 , 0.9527207850133809 )( 0.009284818067754079 , 0.9528991971454059 )( 0.009535759096612296 , 0.9528991971454059 )( 0.009535759096612296 , 0.9532560214094559 )( 0.009535759096612296 , 0.9552185548617306 )( 0.009786700125470515 , 0.9552185548617306 )( 0.009786700125470515 , 0.9557537912578056 )( 0.010288582183186951 , 0.9557537912578056 )( 0.01053952321204517 , 0.9557537912578056 )( 0.01053952321204517 , 0.9561106155218555 )( 0.010790464240903387 , 0.9561106155218555 )( 0.010790464240903387 , 0.9564674397859054 )( 0.011292346298619825 , 0.9564674397859054 )( 0.011292346298619825 , 0.9568242640499554 )( 0.011543287327478042 , 0.9568242640499554 )( 0.011543287327478042 , 0.9571810883140054 )( 0.011794228356336261 , 0.9571810883140054 )( 0.011794228356336261 , 0.9586083853702052 )( 0.01204516938519448 , 0.9586083853702052 )( 0.01204516938519448 , 0.9591436217662801 )( 0.012296110414052697 , 0.9591436217662801 )( 0.012296110414052697 , 0.95950044603033 )( 0.012547051442910916 , 0.95950044603033 )( 0.012547051442910916 , 0.959678858162355 )( 0.012797992471769134 , 0.959678858162355 )( 0.012797992471769134 , 0.960035682426405 )( 0.012797992471769134 , 0.960392506690455 )( 0.013048933500627352 , 0.960392506690455 )( 0.013048933500627352 , 0.9607493309545049 )( 0.013048933500627352 , 0.9614629794826048 )( 0.013299874529485571 , 0.9614629794826048 )( 0.013299874529485571 , 0.9636039250669045 )( 0.013801756587202008 , 0.9636039250669045 )( 0.013801756587202008 , 0.9646743978590544 )( 0.014052697616060227 , 0.9646743978590544 )( 0.014052697616060227 , 0.9652096342551294 )( 0.014303638644918444 , 0.9652096342551294 )( 0.014303638644918444 , 0.9653880463871544 )( 0.014554579673776663 , 0.9653880463871544 )( 0.014554579673776663 , 0.9659232827832293 )( 0.015056461731493099 , 0.9659232827832293 )( 0.015056461731493099 , 0.9664585191793041 )( 0.015307402760351318 , 0.9664585191793041 )( 0.015307402760351318 , 0.9671721677074041 )( 0.015558343789209535 , 0.9671721677074041 )( 0.015558343789209535 , 0.967707404103479 )( 0.01606022584692597 , 0.967707404103479 )( 0.01606022584692597 , 0.968242640499554 )( 0.01631116687578419 , 0.968242640499554 )( 0.01631116687578419 , 0.968421052631579 )( 0.01656210790464241 , 0.968421052631579 )( 0.01656210790464241 , 0.9685994647636039 )( 0.017314930991217063 , 0.9685994647636039 )( 0.017314930991217063 , 0.9689562890276538 )( 0.01756587202007528 , 0.9689562890276538 )( 0.01756587202007528 , 0.9694915254237289 )( 0.0178168130489335 , 0.9694915254237289 )( 0.0178168130489335 , 0.9700267618198037 )( 0.018569636135508157 , 0.9700267618198037 )( 0.018569636135508157 , 0.9702051739518287 )( 0.018820577164366373 , 0.9702051739518287 )( 0.018820577164366373 , 0.9703835860838537 )( 0.01907151819322459 , 0.9703835860838537 )( 0.01907151819322459 , 0.9705619982158786 )( 0.020075282308657464 , 0.9705619982158786 )( 0.020577164366373902 , 0.9705619982158786 )( 0.020577164366373902 , 0.9707404103479037 )( 0.02107904642409034 , 0.9707404103479037 )( 0.02107904642409034 , 0.9712756467439786 )( 0.021580928481806774 , 0.9712756467439786 )( 0.021580928481806774 , 0.9718108831400535 )( 0.021831869510664993 , 0.9718108831400535 )( 0.021831869510664993 , 0.9721677074041035 )( 0.02233375156838143 , 0.9721677074041035 )( 0.02233375156838143 , 0.9727029438001784 )( 0.02258469259723965 , 0.9727029438001784 )( 0.02258469259723965 , 0.9728813559322034 )( 0.023086574654956084 , 0.9728813559322034 )( 0.023086574654956084 , 0.9730597680642283 )( 0.023588456712672522 , 0.9730597680642283 )( 0.023588456712672522 , 0.9734165923282784 )( 0.02383939774153074 , 0.9734165923282784 )( 0.02383939774153074 , 0.9735950044603033 )( 0.024843161856963614 , 0.9735950044603033 )( 0.024843161856963614 , 0.9737734165923283 )( 0.025094102885821833 , 0.9737734165923283 )( 0.025094102885821833 , 0.9743086529884032 )( 0.025595984943538267 , 0.9743086529884032 )( 0.025595984943538267 , 0.9750223015165032 )( 0.026097867001254705 , 0.9750223015165032 )( 0.026097867001254705 , 0.9752007136485281 )( 0.026599749058971143 , 0.9752007136485281 )( 0.027101631116687577 , 0.9752007136485281 )( 0.027101631116687577 , 0.9753791257805531 )( 0.027101631116687577 , 0.975735950044603 )( 0.027101631116687577 , 0.975914362176628 )( 0.027352572145545796 , 0.975914362176628 )( 0.027854454203262234 , 0.975914362176628 )( 0.027854454203262234 , 0.976271186440678 )( 0.028105395232120453 , 0.976271186440678 )( 0.028105395232120453 , 0.976449598572703 )( 0.028607277289836888 , 0.976449598572703 )( 0.028607277289836888 , 0.9768064228367529 )( 0.028858218318695106 , 0.9768064228367529 )( 0.028858218318695106 , 0.9769848349687779 )( 0.029360100376411544 , 0.9769848349687779 )( 0.029360100376411544 , 0.9775200713648529 )( 0.02986198243412798 , 0.9775200713648529 )( 0.02986198243412798 , 0.9778768956289028 )( 0.030614805520702636 , 0.9778768956289028 )( 0.030614805520702636 , 0.9780553077609278 )( 0.030865746549560855 , 0.9780553077609278 )( 0.030865746549560855 , 0.9782337198929527 )( 0.030865746549560855 , 0.9785905441570026 )( 0.03136762860727729 , 0.9785905441570026 )( 0.03136762860727729 , 0.9787689562890276 )( 0.03237139272271016 , 0.9787689562890276 )( 0.03237139272271016 , 0.9789473684210527 )( 0.03262233375156838 , 0.9789473684210527 )( 0.03262233375156838 , 0.9791257805530776 )( 0.03312421580928482 , 0.9791257805530776 )( 0.03312421580928482 , 0.9794826048171276 )( 0.033626097867001256 , 0.9794826048171276 )( 0.033626097867001256 , 0.9796610169491525 )( 0.034127979924717694 , 0.9796610169491525 )( 0.034629861982434125 , 0.9796610169491525 )( 0.03513174404015056 , 0.9796610169491525 )( 0.035633626097867 , 0.9796610169491525 )( 0.035633626097867 , 0.9800178412132025 )( 0.03588456712672522 , 0.9800178412132025 )( 0.03588456712672522 , 0.9807314897413024 )( 0.03613550815558344 , 0.9807314897413024 )( 0.03613550815558344 , 0.9812667261373773 )( 0.036888331242158096 , 0.9812667261373773 )( 0.03814303638644918 , 0.9812667261373773 )( 0.03864491844416562 , 0.9812667261373773 )( 0.03864491844416562 , 0.9814451382694023 )( 0.03889585947302384 , 0.9814451382694023 )( 0.03889585947302384 , 0.9816235504014273 )( 0.03889585947302384 , 0.9819803746654773 )( 0.0396486825595985 , 0.9819803746654773 )( 0.0396486825595985 , 0.9823371989295272 )( 0.04040150564617315 , 0.9823371989295272 )( 0.04040150564617315 , 0.9825156110615522 )( 0.04215809284818068 , 0.9825156110615522 )( 0.04215809284818068 , 0.9828724353256021 )( 0.04341279799247177 , 0.9828724353256021 )( 0.04341279799247177 , 0.9830508474576272 )( 0.0451693851944793 , 0.9830508474576272 )( 0.0451693851944793 , 0.9832292595896521 )( 0.04918444165621079 , 0.9832292595896521 )( 0.04918444165621079 , 0.983586083853702 )( 0.049937264742785446 , 0.983586083853702 )( 0.050439146800501884 , 0.983586083853702 )( 0.05094102885821832 , 0.983586083853702 )( 0.05244667503136763 , 0.983586083853702 )( 0.05244667503136763 , 0.983764495985727 )( 0.053701380175658724 , 0.983764495985727 )( 0.053701380175658724 , 0.983942908117752 )( 0.05846925972396487 , 0.983942908117752 )( 0.05846925972396487 , 0.9841213202497769 )( 0.060225846925972396 , 0.9841213202497769 )( 0.060225846925972396 , 0.984299732381802 )( 0.06097867001254705 , 0.984299732381802 )( 0.06148055207026349 , 0.984299732381802 )( 0.06424090338770388 , 0.984299732381802 )( 0.06424090338770388 , 0.9846565566458519 )( 0.0657465495608532 , 0.9846565566458519 )( 0.0657465495608532 , 0.9848349687778769 )( 0.06624843161856964 , 0.9848349687778769 )( 0.06624843161856964 , 0.9850133809099019 )( 0.06675031367628607 , 0.9850133809099019 )( 0.06725219573400251 , 0.9850133809099019 )( 0.07076537013801756 , 0.9850133809099019 )( 0.07076537013801756 , 0.9853702051739518 )( 0.07151819322459223 , 0.9853702051739518 )( 0.07151819322459223 , 0.9855486173059768 )( 0.07176913425345044 , 0.9855486173059768 )( 0.07227101631116688 , 0.9855486173059768 )( 0.07277289836888332 , 0.9855486173059768 )( 0.07277289836888332 , 0.9857270294380018 )( 0.07728983688833124 , 0.9857270294380018 )( 0.07728983688833124 , 0.9859054415700268 )( 0.07854454203262233 , 0.9859054415700268 )( 0.07854454203262233 , 0.9860838537020518 )( 0.07879548306148056 , 0.9860838537020518 )( 0.0795483061480552 , 0.9860838537020518 )( 0.08030112923462986 , 0.9860838537020518 )( 0.08030112923462986 , 0.9862622658340767 )( 0.08180677540777917 , 0.9862622658340767 )( 0.08180677540777917 , 0.9864406779661017 )( 0.08456712672521957 , 0.9864406779661017 )( 0.08582183186951066 , 0.9869759143621766 )( 0.09360100376411544 , 0.9869759143621766 )( 0.09360100376411544 , 0.9871543264942017 )( 0.09485570890840653 , 0.9871543264942017 )( 0.09485570890840653 , 0.9873327386262266 )( 0.09661229611041405 , 0.9873327386262266 )( 0.09661229611041405 , 0.9875111507582516 )( 0.09786700125470514 , 0.9875111507582516 )( 0.09786700125470514 , 0.9876895628902765 )( 0.0986198243412798 , 0.9876895628902765 )( 0.0986198243412798 , 0.9878679750223015 )( 0.1001254705144291 , 0.9878679750223015 )( 0.1001254705144291 , 0.9880463871543265 )( 0.10062735257214554 , 0.9880463871543265 )( 0.10112923462986198 , 0.9880463871543265 )( 0.1013801756587202 , 0.9880463871543265 )( 0.1013801756587202 , 0.9882247992863514 )( 0.10213299874529486 , 0.9882247992863514 )( 0.10213299874529486 , 0.9884032114183765 )( 0.1028858218318695 , 0.9884032114183765 )( 0.10338770388958594 , 0.9884032114183765 )( 0.10639899623588457 , 0.9884032114183765 )( 0.10639899623588457 , 0.9885816235504015 )( 0.10941028858218318 , 0.9885816235504015 )( 0.10991217063989962 , 0.9885816235504015 )( 0.11267252195734002 , 0.9885816235504015 )( 0.11317440401505646 , 0.9885816235504015 )( 0.11417816813048934 , 0.9885816235504015 )( 0.11417816813048934 , 0.9887600356824264 )( 0.11468005018820578 , 0.9887600356824264 )( 0.11468005018820578 , 0.9889384478144514 )( 0.11744040150564618 , 0.9889384478144514 )( 0.11819322459222083 , 0.9889384478144514 )( 0.11969887076537014 , 0.9889384478144514 )( 0.12020075282308658 , 0.9889384478144514 )( 0.12446675031367628 , 0.9889384478144514 )( 0.12446675031367628 , 0.9892952720785013 )( 0.12823086574654957 , 0.9892952720785013 )( 0.12823086574654957 , 0.9894736842105263 )( 0.12973651191969887 , 0.9894736842105263 )( 0.1302383939774153 , 0.9894736842105263 )( 0.13124215809284817 , 0.9894736842105263 )( 0.13174404015056462 , 0.9894736842105263 )( 0.13324968632371392 , 0.9894736842105263 )( 0.13400250941028857 , 0.9894736842105263 )( 0.13776662484316185 , 0.9894736842105263 )( 0.13776662484316185 , 0.9896520963425512 )( 0.13902132998745295 , 0.9896520963425512 )( 0.13902132998745295 , 0.9898305084745763 )( 0.14153074027603513 , 0.9898305084745763 )( 0.14153074027603513 , 0.9900089206066013 )( 0.14755332496863238 , 0.9900089206066013 )( 0.14855708908406526 , 0.9903657448706512 )( 0.15307402760351319 , 0.9903657448706512 )( 0.15307402760351319 , 0.9905441570026762 )( 0.15633626097867 , 0.9905441570026762 )( 0.15633626097867 , 0.9907225691347011 )( 0.15708908406524466 , 0.9907225691347011 )( 0.1575909661229611 , 0.9907225691347011 )( 0.16110414052697616 , 0.9907225691347011 )( 0.16260978670012546 , 0.9907225691347011 )( 0.16537013801756587 , 0.9907225691347011 )( 0.16612296110414052 , 0.9907225691347011 )( 0.16662484316185697 , 0.9907225691347011 )( 0.16662484316185697 , 0.9909009812667261 )( 0.17038895859473024 , 0.9909009812667261 )( 0.17038895859473024 , 0.9910793933987511 )( 0.17089084065244667 , 0.9910793933987511 )( 0.17089084065244667 , 0.9912578055307761 )( 0.17340025094102887 , 0.9912578055307761 )( 0.17340025094102887 , 0.9914362176628011 )( 0.17691342534504392 , 0.9914362176628011 )( 0.17691342534504392 , 0.991793041926851 )( 0.1779171894604768 , 0.991793041926851 )( 0.1779171894604768 , 0.991971454058876 )( 0.17992471769134252 , 0.991971454058876 )( 0.17992471769134252 , 0.992149866190901 )( 0.1821831869510665 , 0.992149866190901 )( 0.18293601003764115 , 0.992149866190901 )( 0.19096612296110413 , 0.992149866190901 )( 0.1917189460476788 , 0.9923282783229259 )( 0.19498117942283563 , 0.9923282783229259 )( 0.19498117942283563 , 0.992506690454951 )( 0.19799247176913426 , 0.992506690454951 )( 0.19799247176913426 , 0.992685102586976 )( 0.19974905897114179 , 0.992685102586976 )( 0.2002509410288582 , 0.992685102586976 )( 0.2040150564617315 , 0.992685102586976 )( 0.2040150564617315 , 0.9928635147190009 )( 0.20501882057716436 , 0.9928635147190009 )( 0.20501882057716436 , 0.9930419268510259 )( 0.20627352572145546 , 0.9930419268510259 )( 0.2067754077791719 , 0.9930419268510259 )( 0.20903387703889587 , 0.9930419268510259 )( 0.2095357590966123 , 0.9930419268510259 )( 0.21028858218318694 , 0.9930419268510259 )( 0.21028858218318694 , 0.9932203389830508 )( 0.2120451693851945 , 0.9932203389830508 )( 0.2120451693851945 , 0.9933987511150758 )( 0.21279799247176914 , 0.9933987511150758 )( 0.2135508155583438 , 0.9933987511150758 )( 0.2135508155583438 , 0.9935771632471008 )( 0.21656210790464242 , 0.9935771632471008 )( 0.22107904642409035 , 0.9935771632471008 )( 0.22434127979924717 , 0.9935771632471008 )( 0.22434127979924717 , 0.9937555753791257 )( 0.22509410288582182 , 0.9937555753791257 )( 0.22534504391468005 , 0.9939339875111508 )( 0.22936010037641155 , 0.9939339875111508 )( 0.22986198243412798 , 0.9939339875111508 )( 0.23111668757841908 , 0.9939339875111508 )( 0.2316185696361355 , 0.9939339875111508 )( 0.23462986198243413 , 0.9939339875111508 )( 0.23462986198243413 , 0.9941123996431758 )( 0.23889585947302383 , 0.9941123996431758 )( 0.23889585947302383 , 0.9942908117752007 )( 0.23939774153074028 , 0.9942908117752007 )( 0.2529485570890841 , 0.9942908117752007 )( 0.2529485570890841 , 0.9948260481712756 )( 0.25395232120451694 , 0.9948260481712756 )( 0.2544542032622334 , 0.9948260481712756 )( 0.2584692597239649 , 0.9950044603033006 )( 0.25972396486825594 , 0.9950044603033006 )( 0.25972396486825594 , 0.9953612845673506 )( 0.26750313676286075 , 0.9953612845673506 )( 0.26750313676286075 , 0.9955396966993756 )( 0.271267252195734 , 0.9955396966993756 )( 0.271267252195734 , 0.9957181088314006 )( 0.27176913425345045 , 0.9957181088314006 )( 0.2740276035131744 , 0.9957181088314006 )( 0.27452948557089085 , 0.9957181088314006 )( 0.27628607277289835 , 0.9957181088314006 )( 0.27628607277289835 , 0.9958965209634255 )( 0.28431618569636136 , 0.9958965209634255 )( 0.28557089084065246 , 0.9958965209634255 )( 0.2946047678795483 , 0.9958965209634255 )( 0.2946047678795483 , 0.9960749330954505 )( 0.3081555834378921 , 0.9960749330954505 )( 0.3081555834378921 , 0.9962533452274754 )( 0.3111668757841907 , 0.9962533452274754 )( 0.31217063989962357 , 0.9962533452274754 )( 0.3252195734002509 , 0.9962533452274754 )( 0.3252195734002509 , 0.9964317573595004 )( 0.3254705144291092 , 0.9964317573595004 )( 0.3254705144291092 , 0.9966101694915255 )( 0.32772898368883313 , 0.9966101694915255 )( 0.32772898368883313 , 0.9967885816235504 )( 0.3337515683814304 , 0.9967885816235504 )( 0.3342534504391468 , 0.9967885816235504 )( 0.3397741530740276 , 0.9967885816235504 )( 0.3397741530740276 , 0.9969669937555754 )( 0.3462986198243413 , 0.9969669937555754 )( 0.3475533249686324 , 0.9969669937555754 )( 0.3508155583437892 , 0.9969669937555754 )( 0.35131744040150564 , 0.9969669937555754 )( 0.3518193224592221 , 0.9969669937555754 )( 0.35232120451693855 , 0.9969669937555754 )( 0.35834378920953575 , 0.9969669937555754 )( 0.358594730238394 , 0.9971454058876004 )( 0.35984943538268505 , 0.9971454058876004 )( 0.3603513174404015 , 0.9971454058876004 )( 0.36336260978670015 , 0.9971454058876004 )( 0.36336260978670015 , 0.9973238180196253 )( 0.36511919698870765 , 0.9973238180196253 )( 0.36637390213299875 , 0.9973238180196253 )( 0.36637390213299875 , 0.9975022301516503 )( 0.36762860727728985 , 0.9975022301516503 )( 0.3686323713927227 , 0.9975022301516503 )( 0.37641154328732745 , 0.9975022301516503 )( 0.3769134253450439 , 0.9975022301516503 )( 0.37992471769134256 , 0.9975022301516503 )( 0.3806775407779172 , 0.9975022301516503 )( 0.38444165621079046 , 0.9975022301516503 )( 0.3849435382685069 , 0.9975022301516503 )( 0.39974905897114177 , 0.9975022301516503 )( 0.40100376411543287 , 0.9975022301516503 )( 0.4027603513174404 , 0.9975022301516503 )( 0.4032622333751568 , 0.9975022301516503 )( 0.40401505646173147 , 0.9975022301516503 )( 0.40526976160602257 , 0.9975022301516503 )( 0.4117942283563363 , 0.9975022301516503 )( 0.4117942283563363 , 0.9976806422836753 )( 0.41530740276035133 , 0.9976806422836753 )( 0.416060225846926 , 0.9976806422836753 )( 0.41982434127979923 , 0.9976806422836753 )( 0.4203262233375157 , 0.9976806422836753 )( 0.4228356336260979 , 0.9976806422836753 )( 0.42358845671267253 , 0.9976806422836753 )( 0.4406524466750314 , 0.9976806422836753 )( 0.4406524466750314 , 0.9978590544157002 )( 0.4411543287327478 , 0.9978590544157002 )( 0.4411543287327478 , 0.9980374665477253 )( 0.44366373902133 , 0.9980374665477253 )( 0.44366373902133 , 0.9982158786797503 )( 0.44742785445420324 , 0.9982158786797503 )( 0.4481806775407779 , 0.9982158786797503 )( 0.45972396486825595 , 0.9982158786797503 )( 0.4604767879548306 , 0.9982158786797503 )( 0.46800501882057716 , 0.9982158786797503 )( 0.4687578419071518 , 0.9982158786797503 )( 0.46925972396486826 , 0.9982158786797503 )( 0.4697616060225847 , 0.9982158786797503 )( 0.4700125470514429 , 0.9982158786797503 )( 0.47051442910915936 , 0.9982158786797503 )( 0.5036386449184441 , 0.9982158786797503 )( 0.5041405269761606 , 0.9982158786797503 )( 0.5063989962358846 , 0.9982158786797503 )( 0.506900878293601 , 0.9982158786797503 )( 0.5076537013801756 , 0.9982158786797503 )( 0.5081555834378921 , 0.9982158786797503 )( 0.5096612296110414 , 0.9982158786797503 )( 0.5101631116687578 , 0.9982158786797503 )( 0.5146800501882057 , 0.9982158786797503 )( 0.5176913425345044 , 0.9982158786797503 )( 0.5181932245922208 , 0.9982158786797503 )( 0.5214554579673777 , 0.9982158786797503 )( 0.5224592220828106 , 0.9982158786797503 )( 0.526474278544542 , 0.9982158786797503 )( 0.5274780426599749 , 0.9989295272078501 )( 0.5365119196988708 , 0.9989295272078501 )( 0.5370138017565872 , 0.9989295272078501 )( 0.5380175658720201 , 0.9989295272078501 )( 0.5380175658720201 , 0.9991079393398751 )( 0.5417816813048933 , 0.9991079393398751 )( 0.5422835633626097 , 0.9991079393398751 )( 0.5485570890840652 , 0.9991079393398751 )( 0.5500627352572146 , 0.9991079393398751 )( 0.5573400250941029 , 0.9991079393398751 )( 0.5578419071518194 , 0.9991079393398751 )( 0.5606022584692597 , 0.9991079393398751 )( 0.5613550815558344 , 0.9991079393398751 )( 0.5618569636135509 , 0.9991079393398751 )( 0.5636135508155583 , 0.9991079393398751 )( 0.5641154328732748 , 0.9991079393398751 )( 0.5651191969887076 , 0.9991079393398751 )( 0.566624843161857 , 0.9991079393398751 )( 0.570138017565872 , 0.9991079393398751 )( 0.5706398996235884 , 0.9991079393398751 )( 0.5877038895859473 , 0.9991079393398751 )( 0.5882057716436637 , 0.9991079393398751 )( 0.5937264742785445 , 0.9991079393398751 )( 0.594228356336261 , 0.9991079393398751 )( 0.5949811794228357 , 0.9991079393398751 )( 0.5954830614805521 , 0.9991079393398751 )( 0.6070263488080301 , 0.9991079393398751 )( 0.6075282308657466 , 0.9991079393398751 )( 0.609284818067754 , 0.9991079393398751 )( 0.6097867001254705 , 0.9991079393398751 )( 0.613801756587202 , 0.9991079393398751 )( 0.6143036386449184 , 0.9991079393398751 )( 0.6158092848180677 , 0.9991079393398751 )( 0.6163111668757842 , 0.9991079393398751 )( 0.6183186951066499 , 0.9991079393398751 )( 0.6183186951066499 , 0.9992863514719 )( 0.6268506900878293 , 0.9992863514719 )( 0.6283563362609786 , 0.9992863514719 )( 0.6288582183186952 , 0.9992863514719 )( 0.6358845671267253 , 0.9992863514719 )( 0.6393977415307402 , 0.9992863514719 )( 0.6466750313676286 , 0.9992863514719 )( 0.6466750313676286 , 0.9994647636039251 )( 0.6474278544542033 , 0.9994647636039251 )( 0.6479297365119197 , 0.9994647636039251 )( 0.6690087829360101 , 0.9994647636039251 )( 0.6695106649937265 , 0.9994647636039251 )( 0.6777917189460477 , 0.9994647636039251 )( 0.6782936010037641 , 0.9994647636039251 )( 0.6858218318695106 , 0.9994647636039251 )( 0.6863237139272271 , 0.9994647636039251 )( 0.6928481806775407 , 0.9994647636039251 )( 0.6936010037641155 , 0.9994647636039251 )( 0.6963613550815558 , 0.9994647636039251 )( 0.6968632371392722 , 0.9994647636039251 )( 0.6978670012547051 , 0.9994647636039251 )( 0.7189460476787954 , 0.9994647636039251 )( 0.719447929736512 , 0.9994647636039251 )( 0.7239648682559598 , 0.9994647636039251 )( 0.7247176913425345 , 0.9994647636039251 )( 0.736762860727729 , 0.9994647636039251 )( 0.7375156838143037 , 0.9994647636039251 )( 0.7412797992471769 , 0.9994647636039251 )( 0.7417816813048933 , 0.9994647636039251 )( 0.7445420326223338 , 0.9994647636039251 )( 0.7455457967377667 , 0.9994647636039251 )( 0.7535759096612296 , 0.9994647636039251 )( 0.7540777917189461 , 0.9994647636039251 )( 0.7590966122961104 , 0.9994647636039251 )( 0.7595984943538269 , 0.9994647636039251 )( 0.7658720200752823 , 0.9994647636039251 )( 0.7663739021329987 , 0.9994647636039251 )( 0.7691342534504392 , 0.9994647636039251 )( 0.7696361355081556 , 0.9994647636039251 )( 0.7708908406524467 , 0.9994647636039251 )( 0.7708908406524467 , 0.9996431757359501 )( 0.7756587202007528 , 0.9996431757359501 )( 0.7761606022584693 , 0.9996431757359501 )( 0.7831869510664994 , 0.9996431757359501 )( 0.7836888331242158 , 0.9996431757359501 )( 0.8145545796737766 , 0.9996431757359501 )( 0.8150564617314932 , 0.9996431757359501 )( 0.8336260978670013 , 0.9996431757359501 )( 0.8343789209535759 , 0.9996431757359501 )( 0.8361355081555835 , 0.9996431757359501 )( 0.8366373902132999 , 0.9996431757359501 )( 0.8466750313676286 , 0.9996431757359501 )( 0.8471769134253451 , 0.9996431757359501 )( 0.8486825595984944 , 0.9996431757359501 )( 0.8491844416562108 , 0.9996431757359501 )( 0.849435382685069 , 0.9996431757359501 )( 0.849435382685069 , 0.999821587867975 )( 0.852948557089084 , 0.999821587867975 )( 0.8537013801756588 , 0.999821587867975 )( 0.8617314930991217 , 0.999821587867975 )( 0.8617314930991217 , 1.0 )( 0.8737766624843162 , 1.0 )( 0.8742785445420326 , 1.0 )( 0.8755332496863237 , 1.0 )( 0.8765370138017566 , 1.0 )( 0.880552070263488 , 1.0 )( 0.8813048933500628 , 1.0 )( 0.8860727728983688 , 1.0 )( 0.8865746549560853 , 1.0 )( 0.88732747804266 , 1.0 )( 0.8878293601003764 , 1.0 )( 0.888582183186951 , 1.0 )( 0.8900878293601003 , 1.0 )( 0.895357590966123 , 1.0 )( 0.8963613550815558 , 1.0 )( 0.896612296110414 , 1.0 )( 0.8971141781681304 , 1.0 )( 0.9041405269761607 , 1.0 )( 0.904642409033877 , 1.0 )( 0.9111668757841908 , 1.0 )( 0.9116687578419072 , 1.0 )( 0.9227101631116688 , 1.0 )( 0.9232120451693852 , 1.0 )( 0.9249686323713927 , 1.0 )( 0.9254705144291092 , 1.0 )( 0.9304893350062735 , 1.0 )( 0.9312421580928482 , 1.0 )( 0.9322459222082811 , 1.0 )( 0.9327478042659975 , 1.0 )( 0.933249686323714 , 1.0 )( 0.9337515683814304 , 1.0 )( 0.9375156838143036 , 1.0 )( 0.9380175658720201 , 1.0 )( 0.9407779171894605 , 1.0 )( 0.9412797992471769 , 1.0 )( 0.9415307402760351 , 1.0 )( 0.942534504391468 , 1.0 )( 0.9432873274780427 , 1.0 )( 0.9440401505646173 , 1.0 )( 0.9450439146800502 , 1.0 )( 0.9490589711417817 , 1.0 )( 0.9495608531994981 , 1.0 )( 0.954077791718946 , 1.0 )( 0.9545796737766625 , 1.0 )( 0.9683814303638645 , 1.0 )( 0.9693851944792974 , 1.0 )( 0.970138017565872 , 1.0 )( 0.9708908406524467 , 1.0 )( 0.9726474278544542 , 1.0 )( 0.9734002509410289 , 1.0 )( 0.9774153074027604 , 1.0 )( 0.978168130489335 , 1.0 )( 0.9794228356336261 , 1.0 )( 0.9799247176913425 , 1.0 )( 0.9856963613550815 , 1.0 )( 0.986198243412798 , 1.0 )( 0.9914680050188206 , 1.0 )( 0.991969887076537 , 1.0 )( 0.9974905897114178 , 1.0 )( 1.0 , 1.0 ) 
